Price of Anarchy of First-Price Auctions in Agentic Markets

An agentic market is a decentralized serving-time market where AI agents bid to claim each user prompt. An agent's bid is based on its expected value for the prompt, which is the expectation of the reward for its response minus its inference costs. First-price auctions (FPAs), in which the highest bidder pays its bid and receives the prompt, are a natural way to allocate prompts in such a market, since they are simple and transparent to run, and do not require central knowledge of private capabilities and costs. However, FPAs are not truthful: participants may bid less than their true value in the hope of a larger profit, and the prompt may then be allocated to someone other than the bidder who values it the most. This welfare loss is quantified by the $\textit{price-of-anarchy}$ (PoA). In this paper, we argue that agentic markets are likely to possess features that reduce the price-of-anarchy. The first is a $\textit{competitive floor}$, which occurs when multiple bidders usually value the prompt above some baseline share of the optimal welfare (e.g., because the best models are often distilled into cheaper alternatives, which perform similarly). We show that competition among them then limits the welfare loss, which can be driven to zero as the floor rises. The second feature is $\textit{near-independence}$ of values after conditioning on the prompt, which occurs when most of the predictable variation in the expected value is determined by the difficulty of the prompt. As the value distribution approaches conditional independence, we can derive an efficiency guarantee that approaches a factor of $1 - 1/e^2$ of the optimal welfare. Thus, both features give rise to welfare lower bounds that are significantly better than the well-known general case of $1 - 1/e$. We validate these results empirically using auctions with strategic bidders simulated on the EmbedLLM prompt routing dataset.

==> tikz/poa_style.tex <==
% Shared plot style for the TikZ figures in tikz/.
% Self-guarding: each figure file inputs this, but it only executes once.
%
% Requires: \usepackage{pgfplots}, \pgfplotsset{compat=1.18},
%           \usepgfplotslibrary{groupplots}

\ifdefined\poastyleloaded\else
\def\poastyleloaded{1}

\definecolor{poagreen}{RGB}{76,145,96}
\definecolor{poared}{RGB}{196,84,84}
\definecolor{poanavy}{RGB}{40,62,125}
% Okabe-Ito colorblind-safe pair (blue / vermillion); also distinct in grayscale
\definecolor{poablue}{RGB}{0,114,178}
\definecolor{poaverm}{RGB}{213,94,0}

\pgfplotsset{
  poaaxis/.style={
    axis line style={black!80, line width=0.4pt},
    tick align=outside,
    tick style={black!80, line width=0.4pt},
    grid=both,
    major grid style={black!22, dotted, line width=0.4pt},
    minor grid style={black!12, dotted, line width=0.3pt},
    label style={font=\scriptsize},
    tick label style={font=\scriptsize},
    title style={font=\scriptsize, yshift=1pt},
    scaled y ticks=false,
    y tick label style={/pgf/number format/fixed},
    legend cell align=left,
    legend style={
      font=\scriptsize,
      fill=white,
      fill opacity=0.9,
      text opacity=1,
      draw=black!30,
      rounded corners=1pt,
      inner sep=2pt,
      row sep=-1.5pt,
    },
  },
  poaline/.style={line width=0.9pt, mark size=1.3pt},
}

\fi

